Provably Efficient Online Hyperparameter Optimization with Population-Based Bandits

Many of the recent triumphs in machine learning are dependent on well-tuned hyperparameters. This is particularly prominent in reinforcement learning (RL) where a small change in the configuration can lead to failure. Despite the importance of tuning hyperparameters, it remains expensive and is often done in a naive and laborious way. A recent solution to this problem is Population Based Training (PBT) which updates both weights and hyperparameters in a single training run of a population of agents. PBT has been shown to be particularly effective in RL, leading to widespread use in the field. However, PBT lacks theoretical guarantees since it relies on random heuristics to explore the hyperparameter space. This inefficiency means it typically requires vast computational resources, which is prohibitive for many small and medium sized labs. In this work, we introduce the first provably efficient PBT-style algorithm, Population-Based Bandits (PB2). PB2 uses a probabilistic model to guide the search in an efficient way, making it possible to discover high performing hyperparameter configurations with far fewer agents than typically required by PBT. We show in a series of RL experiments that PB2 is able to achieve high performance with a modest computational budget.

==> TVGP_Theoretical_Analysis.tex <==

\paragraph{Regret.}

A natural performance metric in this context is cumulative regret,
the loss in reward due to not knowing the maximum points of the black-box
function beforehand. Suppose the unknown function is f, its maximum
point $\bx^{*}=\arg\max_{\bx\in D}f(\bx)$. For our choice $\bx_{t}$
in iteration $t$, we incur instantaneous regret $r_{t}=f\left(\bx^{*}\right)-f\left(\bx_{t}\right)$.
The cumulative regret $R_{T}$ after $T$ iterations is the sum of
instantaneous regrets: $R_{T}=\sum_{t=1}^{T}r_{t}$. A desirable asymptotic
property of an algorithm is to be no-regret: $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.
Note that neither $r_{t}$ nor $R_{T}$ are ever revealed to the algorithm.

\subsection{Convergence Analysis}
\label{sec:convergence}

We aim to minimize the cumulative regret $R_{T}$ by sequentially suggest
a $\bx_{t}$ to be used in each iteration $t$. We shall derive the
upper bound in the cumulative regret and show that it asymptoticaly
goes to zero as $T$ increases, i.e., $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.

We make the following smoothness assumption to derive the regret bound
of the proposed algorithm.

\paragraph{Assumptions.}
We will assume that the kernel $k$ is such that a (strict) subset
of the following statements hold for some $\left(a,b\right)$ and
all $L\ge0$.
\begin{enumerate}
\item The time kernel satisfies $1-k_{time}(t,t')\le\omega\left|t-t'\right|$
for some $\omega\in\left[0,1\right]$ and for any $t,t'\in\mathcal{T}$.
\item The joint kernel satisfies for $k=1,...,K,$
\begin{align}
\forall L & \ge0,t\le\mathcal{T},p(\sup\left|\frac{\partial f_{t}(\bbeta)}{\partial\bbeta^{(k)}}\right|\le L)\le ae^{-\left(L/b\right)^{2}}.\label{eq:Lipschitz_assumption}
\end{align}
\end{enumerate}
The assumption 1 is achieved by using a time-varying kernel $k_{time}(t,t')=\left(1-\omega\right)^{\frac{|t-t'|}{2}}$
\citep{bogunovic2016time} while assumption 2 is from the fact the functions are smooth.
\begin{lemma}
\label{lem:Lipschitz_bound}Let $L_{t}=b\sqrt{\log3da\frac{\pi_{t}}{\delta}})$
where $\sum_{t=1}^{T}\frac{1}{\pi_{t}}=1$, we have with probability
$1-\frac{\delta}{3},$
\begin{align}
\left|f_{t}(\bx)-f_{t}(\bx')\right| & \le L_{t}||\bx-\bx'||_{1},\forall t,\bx,\bx'\in D\label{eq:Lipschitz_Lt}
\end{align}
\end{lemma}

\begin{proof}
Using the Lipschitz assumption in Eq. (\ref{eq:Lipschitz_assumption})
and the union bound over $j=1,...,d$, the event corresponding to
a single time in Eq. (\ref{eq:Lipschitz_Lt}) will hold with the probability
at least $1-da\exp\left(-\frac{L_{t}^{2}}{b^{2}}\right)=1-\frac{\delta}{3\pi_{t}}$.
Taking the union bound over $t$, we get $1-\sum_{t=1}^{T}da\exp\left(-\frac{L_{t}^{2}}{b^{2}}\right)=1-\sum_{t=1}^{T}\frac{\delta}{3\pi_{t}}=1-\frac{\delta}{3}$
since $\sum_{t=1}^{T}\frac{1}{\pi_{t}}=1$.
\end{proof}
We below define a discretization which serves as a tool for proving
the theorem, but it is not used in the implementation.
\begin{lemma}
\label{lem:bound_discretization}We define a discretization $D_{t}\subset D\subseteq[0,r]^{d}$
of size $(\tau_{t})^{d}$ satisfying $||\bx-\left[\bx\right]_{t}||_{1}\le\frac{d}{\tau_{t}},\forall\bx\in D$
where $\left[\bx\right]_{t}$ denotes the closest point in $D_{t}$
to $\bx$. By choosing $\tau_{t}=\frac{t^{2}}{L_{t}d}=rdbt^{2}\sqrt{\log\left(3da\pi_{t}/\delta\right)}$,
we have
\begin{align*}
|f_{t}(\bx)-f_{t}(\left[\bx\right]_{t})| & \le\frac{1}{t^{2}}
\end{align*}
\end{lemma}

\begin{proof}
Using the discretization assumption and the Lipschitz continuity in
Lemma \ref{lem:Lipschitz_bound}, we have
\begin{align*}
\left|f_{t}(\bx)\text{\textminus}f_{t}(\left[\bx\right]_{t})\right| & \le L_{t}||\bx-\left[\bx\right]_{t}||_{1}\le\frac{L_{t}d}{\tau_{t}}
\end{align*}
By setting $\tau_{t}=\frac{t^{2}}{L_{t}d}$, we have that $\left|f_{t}(\bx)-f_{t}(\left[\bx\right]_{t})\right|\le\frac{1}{t^{2}}$.
\end{proof}
We note that a uniformly-spaced grid suffices to ensure the discretization
holds.
\begin{lemma}
\label{lem:bound_fx_mux}Let $\kappa_{t}\ge2\log\frac{3\pi_{t}}{\delta}+2d\log\left(rdbt^{2}\sqrt{\log\frac{3da\pi_{t}}{2\delta}}\right)$
where $\sum_{t=1}^{T}\pi_{t}^{-1}=1$, then with probability at least
$1-\frac{\delta}{3}$, we have
\begin{align*}
|f_{t}(\bx_{t})-\mu_{t}(\bx_{t})|\le & \sqrt{\kappa_{t}}\sigma_{t}(\bx_{t}),\forall t,\forall\bx\in\mathcal{D}.
\end{align*}
\end{lemma}

\begin{proof}
Note that conditioned on the outputs $(y_{1},...,y_{t-1})$, the
sampled points $(\bx_{1},...,\bx_{t})$ are deterministic, and $f_{t}(\bx_{t})\sim\mathcal{N}\left(\mu_{t}(\bx_{t}),\sigma_{t}^{2}(\bx_{t})\right)$.
Using Gaussian tail bounds \cite{wainwright2015chapter}, a random
variable $f\sim\mathcal{N}(\mu,\sigma^{2})$ is within $\sqrt{\kappa}\sigma$
of $\mu$ with probability at least $1-\exp\left(-\frac{\kappa}{2}\right)$. Therefore, we first claim that if $\kappa_{t}\ge2\log\frac{3\pi_{t}}{\delta}$
then the selected points $\left\{ \bx_{t}\right\} _{t=1}^{T}$ satisfy
the confidence bounds with probability at least $1-\frac{\delta}{3}$
\begin{align}
\left|f_{t}(\bx_{t})-\mu_{t}(\bx_{t})\right| & \le\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t}),\forall t.\label{eq:bound_selected_xt}
\end{align}

This is true because the confidence bound for individual $\bx_{t}$
will hold with probability at least $1-\frac{\delta}{3\pi_{t}}$ and
taking union bound over $\forall t$ will lead to $1-\frac{\delta}{3}$.

We above show that the bound is applicable for the selected points
$\left\{ \bx_{t}\right\} _{t=1}^{T}$. To ensure that the bound is
applicable for all points in the domain $D_{t}$ and $\forall t$,
we can set $\kappa_{t}\ge2\log\frac{3|D_{t}|\pi_{t}}{\delta}$ where
$\sum_{t=1}^{T}\pi_{t}^{-1}=1$ e.g.$\pi_{t}=\frac{\pi^{2}t^{2}}{6}$
\begin{align}
p(\left|f_{t}\left(\bx_{t}\right)-\mu_{t}\left(\bx_{t}\right)\right| & \le\sqrt{\kappa_{t}}\sigma_{t}\left(\bx_{t}\right)\ge1-|D_{t}|\sum_{t=1}^{T}\exp\left(-\kappa_{t}/2\right)=1-\frac{\delta}{3}\label{eq:bound_all_Dt}
\end{align}

By discretizing the domain $D_{t}$ in Lemma \ref{lem:bound_discretization},
we have a connection to the cardinality of the domain that $|D_{t}|=(\tau_{t})^{d}=\left(rdbt^{2}\sqrt{\log\left(3da\pi_{t}/\delta\right)}\right)^{d}$.
 Therefore, we need to set $\kappa_{t}$ such that both conditions
in Eq. (\ref{eq:bound_selected_xt}) and Eq. (\ref{eq:bound_all_Dt})
are satisfied. We simply take a sum of them and get $\kappa_{t}\ge2\log\frac{3\pi_{t}}{\delta}+2d\log\left(rdbt^{2}\sqrt{\log\frac{3da\pi_{t}}{2\delta}}\right)$
.
\end{proof}


\paragraph{Mutual Information:}

The mutual information is one of the key quantites in the regret bound for GP-UCB, originally derived by \cite{gp_ucb}. In this setting, the mutual information is defined as $\tilde{\idenmat}(f_{T};y_{T})=\frac{1}{2}\log\det\left(\idenmat_{T}+\sigma_{f}^{-2}\tilde{K}_{T}\right)$
and the maximum information gain is as $\tilde{\gamma}_{T}:=\max\tilde{\idenmat}({\bf f}_{T};\by_{T})$
where ${\bf f}_{T}:=f_{T}(\bx_{T})=\left(f_{1}(\bx_{1}),...,f_{T}(\bx_{T})\right)$
for the time variant GP $f$. 

We will now show that $\tilde{\gamma}_{T}\le\left(\frac{T}{\tilde{N}}+1\right)\left(\gamma_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)$
where we note that this bound is tighter than the result presented
in the original paper by \cite{bogunovic2016time} ($\tilde{N}^{5/2}\le\tilde{N}^{3}$)
and we have considered noise variance $\sigma_{f}^{-2}$.
\begin{lemma}
\label{lem:Mirsky=002019s-theorem}(Mirsky\textquoteright s theorem
{[}\cite{horn2012matrix}, Cor. 7.4.9.3{]}) For any matrices $U$
and $V$ of size $\tilde{N}\times\tilde{N}$, and any unitarily invariant
norm $|||\cdot|||$, we have 
\begin{align*}
|||\textrm{diag}(\lambda_{1}(U),...,\lambda_{\tilde{N}}(U))-\textrm{diag}(\lambda_{1}(V),...,\lambda_{\tilde{N}}(V))||| & \le|||U-V|||
\end{align*}
where $\lambda_{i}(\cdot)$ is the $i$-th largest eigenvalue.
\end{lemma}


\begin{lemma}
\label{lem:bound_MIG_timevarying}Let $\omega$ be the forgetting-remembering
trade-off parameter and consider the kernel for time $1-K_{time}(t,t')\le\omega\left|t-t'\right|$,
we show that
\begin{align*}
\tilde{\gamma}_{T} & \le\left(\frac{T}{\tilde{N}}+1\right)\left(\gamma_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)
\end{align*}
\end{lemma}

\begin{proof}
We bound the mutual information with time variations by connecting
to the original case (without time variations, \citep{gp_ucb}).
We shall split the time steps $\left\{ 1,...,T\right\} $ into $T/\tilde{N}$
blocks of length $\tilde{N}$, such that within each block the function
$f_{i}$ does not vary significantly. We assume for the time being
that $T/\tilde{N}$ is an integer, and then handle the general case.

We bound the time-varying maximum information gain for each block
$i$-th as $\tilde{\gamma}^{i}:=\max\tilde{\idenmat}^{i}({\bf f}^{i};\by^{i})$
where $\by^{i}=[y_{1},...,y_{\tilde{N}}]$ contains the observations
in the $i$-th blocks and analogous design for ${\bf f}^{i}$, we
write the relevant covariance matrix as
\begin{align*}
\tilde{K}^{i}=K^{i}\circ K_{time}^{i} & =K^{i}+A^{i}
\end{align*}
where $\circ$ denotes the Hadamard product, $K_{time}^{i}=\left[(1-\omega)^{\frac{\left|t-t'\right|}{2}}\right]$,
$A^{i}=K^{i}\circ\left(K_{time}^{i}-\mathbf{1}_{\tilde{N}}\right)$
and $\mathbf{1}_{\tilde{N}}$ is the matrix of one of size $\tilde{N}$.
Each covariance matrix $\tilde{K}^{i},K^{i}$ and $K_{time}^{i}$
will have the same dimension of $\tilde{N}\times\tilde{N}$. We have
each entry in $K^{i}$ is bounded $[0,1]$ and the absolute value
of each entry in $K_{time}^{i}-\mathbf{1}_{\tilde{N}}$ is bounded
by $1-\left(1-\omega\right)^{\frac{\left|i-j\right|}{2}}\le\omega\left|i-j\right|$.

Therefore, we can bound the Frobenius norm of $||A^{i}||_{F}\le\sum_{i,j}\left(i-j\right)^{2}\omega^{2}=\frac{1}{6}\tilde{N}^{2}\left(\tilde{N}^{2}-1\right)\omega^{2}\le\tilde{N}^{4}\omega^{2}$
using a standard double summation formula.

Let $U=K^{i}+A^{i}$ and $V=K^{i}$, we define $\Delta_{k}^{i}=\lambda_{k}\left(\tilde{K}^{i}\right)-\lambda_{k}\left(K^{i}\right)$,
we have
\begin{align*}
\sum_{j=1}^{\tilde{N}}\left(\Delta_{j}^{i}\right)^{2} & =\sum_{j=1}^{\tilde{N}}\left(\lambda_{j}\left(\tilde{K}^{i}\right)-\lambda_{j}\left(K^{i}\right)\right)^{2}\\
 & =||diag\left(\lambda_{1}\left(\tilde{K}^{i}\right),...,\lambda_{\tilde{N}}\left(\tilde{K}^{i}\right)\right)-diag\left(\lambda_{1}\left(K^{i}\right),...,\lambda_{\tilde{N}}\left(K^{i}\right)\right)||_{F}^{2}\le||A_{\tilde{N}}||_{F}^{2}\le\tilde{N}^{4}\omega^{2}
\end{align*}
where we have utilized Lem. \ref{lem:Mirsky=002019s-theorem}. We
now bound the maximum information gain defined in each block $\tilde{\gamma}^{i}$
and connect it to the standard (time invariant) maximum information
gain $\gamma^{i}$ shown in\cite{gp_ucb}
\begin{align}
\tilde{\gamma}^{i}= & \frac{1}{2}\log\det\left(\idenmat_{\tilde{N}\times\tilde{N}}+\sigma^{-2}\left(\tilde{K}^{i}\right)\right)\nonumber \\
= & \sum_{i=1}^{\tilde{N}}\log\left(1+\sigma^{-2}\lambda_{i}\left(K^{i}+A^{i}\right)\right)=\sum_{i=1}^{\tilde{N}}\log\left(1+\sigma^{-2}\lambda_{i}\left(K^{i}\right)+\sigma^{-2}\Delta_{k}^{i}\right)\nonumber \\
\le & \sum_{i=1}^{\tilde{N}}\log\left(1+\sigma^{-2}\lambda_{i}\left(K^{i}\right)\right)+\sum_{i=1}^{\tilde{N}}\log\left(1+\sigma^{-2}\Delta_{k}^{i}\right)\label{eq:log(1_a_b)}\\
= & \gamma_{\tilde{N}}+\sum_{i=1}^{\tilde{N}}\log\left(1+\sigma^{-2}\lambda_{i}\Delta_{k}^{i}\right)\le\gamma_{\tilde{N}}+\tilde{N}\log\left(1+\sigma^{-2}\frac{1}{\tilde{N}}\sum_{i=1}^{\tilde{N}}\Delta_{k}^{i}\right)\label{eq:jensen_delta_i_k}\\
\le & \gamma_{\tilde{N}}+\tilde{N}\log\left(1+\sigma^{-2}\tilde{N}^{3/2}\omega\right)\label{eq:MIG_log_sum_delta_ik}\\
\le & \gamma_{\tilde{N}}+\sigma^{-2}\tilde{N}^{5/2}\omega\label{eq:MIG_log(1_x)}
\end{align}
where Eq. (\ref{eq:log(1_a_b)}) is by $\log(1+a+b)\le\log(1+a)+\log(1+b),$
for $a,b>0$. Eq. (\ref{eq:jensen_delta_i_k}) is using Jensen inequality
for $\log\left(1+x\right)$. In Eq. (\ref{eq:MIG_log_sum_delta_ik}),
we utilize the inequality that $\sum_{i=1}^{\tilde{N}}\Delta_{k}^{i}\le\sqrt{\tilde{N}}\sqrt{\sum_{i=1}^{\tilde{N}}\Delta_{k}^{i}}\le\sqrt{\tilde{N}}\tilde{N}^{2}\omega$.
In Eq. (\ref{eq:MIG_log(1_x)}), we utilize $\log(1+x)\le x$ for
$\forall x>-1$.

Using the chain rule for mutual information and the fact that the
noise sequence $\left\{ \epsilon_{t}\right\} _{t=1}^{T}$ where $y_{t}=f_{t}(\bx_{t})+\epsilon_{t}$
is independent, we have
\begin{align*}
\tilde{\idenmat}_{T}\left(f_{T},y_{T}\right) & \le\sum_{i=1}^{T/\tilde{N}}\tilde{\idenmat}^{i}\left({\bf f}^{i};\by^{i}\right)
\end{align*}
Maximizing both sides $\tilde{\gamma}_{T}:=\max\tilde{\idenmat}({\bf f}_{T};\by_{T})$,
we have
\begin{align*}
\tilde{\gamma}_{T} & \le\sum_{i=1}^{T/\tilde{N}}\tilde{\gamma}^{i}\le\left(\frac{T}{\tilde{N}}+1\right)\left(\gamma_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)
\end{align*}
where the bounds are similar across blocks $\tilde{\gamma}^{i}\le\gamma_{\tilde{N}}+\frac{1}{\sigma_{f}^{2}}\tilde{N}^{5/2}\omega,\forall i\le\frac{T}{\tilde{N}}$
and the addition of one is for the case when $\frac{T}{\tilde{N}}$
is not an integer.
\end{proof}
In particular, we note that the bound over the maximum information
gain for the time-varying is typically much higher than the standard
(non time-varying setting) due to the fact the time-varying function
$f_{T}$ represents the points of $T$ different random functions,
as opposed to a single function at $T$ different points.
\begin{theorem}
Let the domain $\mathcal{D}\subset[0,r]^{d}$ be compact and convex,
and suppose that the kernel is such that $f\sim GP(0,k)$ is almost
surely continuously differentiable and satisfies Lem. \ref{lem:Lipschitz}
for some $(a,b)$. Fix $\delta\in(0,1)$ and set $\kappa_{T}=2\log\frac{\pi^{2}T^{2}}{2\delta}+2d\log rdbT^{2}\sqrt{\log\frac{da\pi^{2}T^{2}}{2\delta}}$.
Defining $C_{1}=8/\log(1+\sigma_{f}^{2})$, the TV-GP-UCB algorithm
satisfies the following after $T$ time steps:
\begin{align*}
R_{T}=\sum_{t=1}^{T}f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t})\le\sqrt{C_{1}T\kappa_{T}\gamma_{T}}+2 & \le\sqrt{C_{1}T\kappa_{T}\left(\frac{T}{\tilde{N}}+1\right)\left(\gamma_{\tilde{N}}+\tilde{N}^{3}\omega\right)}+2
\end{align*}
with probability at least $1-\delta$, the bound is holds for any
$\tilde{N}\in\left\{ 1,...,T\right\} $.
\end{theorem}

\begin{proof}
For Lem. \ref{lem:bound_fx_mux} and Lem. \ref{lem:bound_discretization}
valid, we need to choose $\kappa_{t}$ such as both conditions are
satisfied. Therefore, we choose $\kappa_{t}$ as the union of them.
This choise of $\tau_{t}$ will lead to $|D_{t}|=(\tau_{t})^{d}=\left(rdbt^{2}\sqrt{\log\left(3da\pi_{t}/\delta\right)}\right)^{d}$.

Let $\bx_{t}^{*}=\arg\max_{\forall\bx}f_{t}(\bx)$, we bound the instantaneous
regret as
\begin{align}
r_{t} & =f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t})\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\textrm{by}\,\textrm{Lem}.\thinspace\ref{lem:bound_fx_mux}\nonumber \\
 & \le\text{\ensuremath{\mu_{t}(\bx_{t}^{*})+\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t}^{*})+\frac{1}{t^{2}}-f_{t}(\bx_{t})}}\,\,\,\,\,\,\textrm{by}\,\textrm{Lem}.\,\ref{lem:bound_discretization}\nonumber \\
 & \le\mu_{t}(\bx_{t})+\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t})+\frac{1}{t^{2}}-f_{t}(\bx_{t})\label{eq:inequality_beta_t_argmax}\\
 & \le2\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t})+\frac{1}{t^{2}}\label{eq:bound_rt}
\end{align}
where in Eq. (\ref{eq:inequality_beta_t_argmax}) we have used the
property that $\mu_{t}(\bx_{t})+\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t})\ge\mu_{t}(\bx_{t}^{*})+\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t}^{*})$
by the definition of selecting $\bx_{t}=\arg\max_{\bx}\mu_{t}(\bx)+\sqrt{\kappa_{t}}\sigma_{t}(\bx)$.

Next, we bound the cumulative regret as
\begin{align}
R_{T}=\sum_{t=1}^{T}r_{t} & \le\sum_{t=1}^{T}\left(2\sqrt{\kappa_{t}}\sigma_{t}(\bx_{t})+\frac{1}{t^{2}}\right)\,\textrm{by\,Eq.\,(\ref{eq:bound_rt})}\nonumber \\
 & \le\sqrt{T\sum_{t=1}^{T}4\kappa_{t}\sigma_{t}^{2}(\bx_{t})}+2\label{eq:R_T_step2}\\
 & \le\sqrt{C_{1}T\kappa_{T}\tilde{\gamma}_{T}}+2\label{eq:Lem54Srinivas}\\
 & \le\sqrt{C_{1}T\kappa_{T}\left(\frac{T}{\tilde{N}}+1\right)\left(\gamma_{\tilde{N}}+\frac{1}{\sigma_{f}^{2}}\tilde{N}^{5/2}\omega\right)}+2.\label{eq:R_T_last_step}
\end{align}
 In Eq. (\ref{eq:R_T_step2}) we have used $\sum_{t=1}^{\infty}\frac{1}{t^{2}}\le\pi^{2}/6\le2$
and $||z||_{1}\le\sqrt{T}||z||_{2}$ for any vector $z\in\mathcal{R}^{T}$.
In Eq. (\ref{eq:Lem54Srinivas}), we make use of Lemma 5.4 of \cite{Srinivas_2010Gaussian}
and the fact that $\kappa_{T}\ge\kappa_{t},\forall t\le T$. In Eq.
(\ref{eq:R_T_last_step}), we utilize Lem. \ref{lem:bound_MIG_timevarying}.

Finally, given the squared exponential (SE) kernel defined, $\gamma_{\tilde{N}}^{SE}=\mathcal{O}(\left[\log T\right]^{d+1})$,
the bound is $R_{T}\le\sqrt{C_{1}T\kappa_{T}\left(\frac{T}{\tilde{N}}+1\right)\left((d+1)\log T+\frac{1}{\sigma_{f}^{2}}\tilde{N}^{5/2}\omega\right)}+2$.
We refer to Theorem 5 in [again, cite Srinivas paper] \cite{Srinivas_2010Gaussian} for the bound
of other common kernels. We note that this bound $R_{T}$ in Eq. (\ref{eq:R_T_last_step})
is tighter than in the original paper \cite{bogunovic2016time} due
to the $\tilde{\gamma}_{T}$ derived in Lem. \ref{lem:bound_MIG_timevarying}
(ours $\tilde{N}^{5/2}\le\tilde{N}^{3}$ \cite{bogunovic2016time}).

The regret bound grows sublinearly with the number of iterations $T$,
i.e., $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$. This bound suggests
that the gap between $f_{t}(\bx_{t})$ and the optimal $f_{t}(\bx_{t}^{*})$
is asymptotically vanished.
\end{proof}

Our theoretical analysis assumed that we know the hyperparameters
of both spatial (lengthscale $\sigma_{l}^{2}$ for squared exponential
kernel) and temporal kernel ($\omega$). Having perfect knowledge
of and other hyperparameters is typically not realistic. The GP perspective
allows us to select them in a principled way by maximizing the GP
marginal likelihood


==> algs_backup.tex <==

\section{Population-Based Bandit Optimization}
\label{sec:pb2}

We now introduce Population-Based Bandit Optimization (PB2). The core structure of the algorithm is similar to PBT. PB2 trains a population of agents in parallel. However, while we still copy \textit{weights} from superior models, the key difference comes in the selection of $x_t^i$. After each agent $i$ completes $t_\mathrm{ready}$ training steps, we store the data $(y_t^i, t, x_t^i)$ in a dataset $D_t$. When it comes to selecting new hyperparamters, $x_{t+1}$, we can use the existing data ($D_t$) to model the function $f_t$ with a GP. 

For the GP kernel we use $\tilde\k = k_{\mathrm{SE}} \circ k^{\mathrm{time}}$, which considers the time varying nature of training a neural network. For the acquisition function, we use Eqn. \ref{eq:gp_bucb_acq}, to capture the reduction in uncertainty for models currently training. As far as we know, this is the first use of a time-varying kernel in the batch setting. Unlike PBT, this allows us to efficiently make use of data from previous trials when selecting new configurations, rather than reverting to a uniform prior, or perturbing existing configurations. The full algorithm is shown in Algorithm \ref{Alg:pb2}. 

{\centering
\scalebox{0.95}{\begin{minipage}{.99\linewidth}
    \begin{algorithm}[H]
    \textbf{Initialize:} Network weights $\{\theta_0^i\}_{i=1}^B$, hyperparameters $\{x_0^i\}_{i=1}^B$, dataset $D_0 = \emptyset$ \\
    \textbf{(in parallel)} \For{$t=1, \ldots, T-1$}{
      1. \textbf{Update Models:} $\theta_{t}^i \leftarrow \mathrm{step}(\theta_{t-1}^i | x_{t-1}^i) $ \; \\
      2. \textbf{Evaluate Models:} $y_t^i = F_t(x_{t}^i)- F_{t-1}(x_{t-1}^i) + \epsilon_t$ for all $i$\;\\
      3. \textbf{Record Data:} $D_t = D_{t-1} \cup \{(y_t^i, t, x_t^i)\}_{i=1}^B$ \;\\
      4. If $t \mod t_{\mathrm{ready}} = 0$: 
      \begin{itemize}
          \item \textbf{Copy weights:} Rank agents, if $\theta^i$ is in the bottom $\lambda\%$ then copy weights $\theta^j$ from the top $\lambda\%$.
          \item \textbf{Select hyperparameters:} Fit a GP model to $D_t$ and select hyper-parameters $x^i_t$ by maximizing equation (\ref{eq:gp_bucb_acq}).
      \end{itemize}}
     \textbf{Return best model.}
     \caption{Population-Based Bandit Optimization (PB2)}
    \label{Alg:pb2}
    \end{algorithm}
\end{minipage}
}}

\noindent Next we present our main theoretical result, showing that PB2 is able to achieve sublinear regret. This is the first such result for a PBT-style algorithm. 
\begin{theorem}
Let the domain $\mathcal{D}\subset[0,r]^{d}$ be compact and convex
where $d$ is the dimension and suppose that the kernel is such that
$f\sim GP(0,k)$ is almost surely continuously differentiable and
satisfies Lipschitz assumptions for some $a,b$. Fix $\delta\in(0,1)$
and set $\beta_{T}=2\log\frac{\pi^{2}T^{2}}{2\delta}+2d\log rdbT^{2}\sqrt{\log\frac{da\pi^{2}T^{2}}{2\delta}}$.
Defining $C_{1}=32/\log(1+\sigma_{f}^{2})$, the PB2 algorithm satisfies
the following regret bound after $T$ time steps with probability at least $1-\delta$:
\begin{align*}
R_{TB}=\sum_{t=1}^{T}f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t})\le & \sqrt{C_{1}T\beta_{T}\left(\frac{T}{\tilde{N}B}+1\right)\left(\gamma_{\tilde{N}B}+\left[\tilde{N}B\right]^{\frac{5}{2}}\omega\right)}+2
\end{align*}
the bound holds for any block length
$\tilde{N}\in\left\{ 1,...,T\right\} $ and $B\ll T$.
\end{theorem}

This result shows the regret for PB2 decreases as we increase the population size $B$. This should be expected, since adding computational resources should benefit final performance (which is equivalent to minimizing regret). When using single agent $B=1$, our bound becomes the time-vaying GP-UCB setting in \cite{bogunovic2016time}. 

This theoretical result is novel and significant in two folds. First, by showing the equivalent between maximizing reward and minimizing the bandit regret, this regret bound quantifies the gap between the optimal reward and the achieved reward (by the selected parameter) that is vanishing. To the best of our knowledge, this is the first kind of convergence guarantee in population-based algorithm. Second, the regret bound extends the result established by \cite{bogunovic2016time} to a more general case of handling parallel setting.

Our approach is advantageous against all existing batch BO approaches \cite{desautels2014parallelizing,gonzalez2016batch} that our PB2 considers optimization in a \textit{single training run} while the existing works need to evaluate using multiple reparations.


%Note that in practice, we use the same fixed \vcom{they used $0.8 \log ( 4\times t)$ so it is not fixed } parameterization for $\beta_t$ as in \cite{bogunovic2016time} \vcom{this sentence could be placed in the experimental setting.}.


==> preliminaries_backup.tex <==

\section{Background} \label{sec:background}
\subsection{Problem Statement} 

In this paper we consider the problem of selecting optimal hyperparameters, $x_t^i$, from a compact, convex subset $\mathcal{D}\in \mathbb{R}^d$. Here the index $i$ refers to the $i$th agent in a population/batch, and we use the subscript $t$ to represent the number of timesteps/epochs/iterations elapsed during the training of a neural network. The Population-Based Training (PBT, \cite{pbt}) algorithm trains a population (or batch) of $B$ agents in parallel. Each agent $i\in B$ has both hyperparameters $x_t^i \in \mathbb{R}^d$ and weights $\theta_t^i$. At every $t_{ready}$ step interval (i.e. if $t \mod t_{ready} = 0$), the agents are ranked and the worst performing agents are replaced with members of the best performing agents ($A \subset B$) as follows:
\begin{itemize}
    \item \textbf{Weights} ($\theta_t^i$): copied from one of the best performing agents, i.e. $\theta_t^j \sim \mathrm{Unif}\{\theta_t^j\}_{j \in A}$.
    \item \textbf{Hyperparameters} ($x_t^i$): with probability $\epsilon$ it uses \textbf{random exploration}, and re-samples from the original distribution, otherwise, it uses \textbf{greedy exploration}, and perturbs one of the best performing agents, i.e $\{x^j * \lambda\}_{j\in A}, \lambda \sim [0.8, 1.2]$. 
\end{itemize}
This leads to the learning of hyperparameter schedules, which mean a single agent can have different configurations during a single training run. 
%\paragraph{Why Minimize Regret?} 

To formalize this problem, let $F_t(x_t)$ be an objective function under a given set of hyperparameters at timestep $t$. An example of $F_t(x_t)$ could be the reward for a deep RL agent. When training for a total of $T$ steps, our goal is to maximize the final reward $F_T(x_T)$. We formulate this problem as optimizing the time-varying black-box reward function $f_t$, over $\mathcal{D}$. Every $t_{\mathrm{ready}}$ steps, we observe and record noisy observations, $y_t = f_t(x_t) + \epsilon_t$, where $\epsilon_t \sim \mathcal{N}(0, \sigma^2\mathbf{I})$ for some fixed $\sigma^2$. The function $f_t$ represents the change in $F_t$ after training for $t_{\mathrm{ready}}$ steps, i.e. $F_t - F_{t-t_\mathrm{ready}}$. We define the best choice at each timestep as $x_t^* = \argmax_{x_t\in\mathcal{D}}f_t(x_t)$, and so the \textbf{regret} of each decision as $r_t = f_t(x_t^*) - f_t(x_t)$. 

\begin{lemma} \label{lem:maxreward_minregret}
Maximizing the final performance $F_T$ of a model with respect to a given hyperparameter schedule $\{x_t\}_{t=1}^T$ is equivalent to maximizing the time-varying black-box function $f_t(x_t)$ and minimizing the corresponding cumulative regret $r_t(x_t)$,
\begin{align}
\max F_T(x_T)= \max \sum^T_{t=1} f_t(x_t) =  \min \sum^T_{t=1} r_t(x_t).
\end{align}
\end{lemma}
%We refer to Sec. \ref{} in the appendix for the proof.
In subsequent sections, we present a time-varying bandit approach which is used to minimize the cumulative regret $R_T = \sum_{t=1}^T r_t$. Lemma \ref{lem:maxreward_minregret} shows this is equivalent to maximizing the final performance/reward of a neural network model (see: Section \ref{sec:theory} for the proof).


\begin{comment}
\subsection{Sublinear Regret for GP-Bandit Optimization}

The GP-UCB algorithm \cite{gp_ucb} draws insights from the bandit literature and selects the next point $x_t$, using an acquisition function known as the upper confidence bound (UCB), as follows:
\begin{equation}
    x_t = \argmax_{x\in \mathcal{D}} \mu_{t-1}(x) + \sqrt{\beta_t} \sigma_{t-1}(x)
\end{equation}

where $\beta_t >0$ is a time dependent trade-off between exploration and exploitation. This can be interpreted as taking $x_t$ to be the maximum point within a confidence interval around $f_t$. \cite{gp_ucb} show for certain $\beta_t$, this algorithm achieves sublinear regret, with $R_T = \mathcal{O}(\sqrt{T\beta_T\gamma_T})$, where $\gamma_T$ is the \textit{maximum information gain} after $T$ rounds, defined as:
\begin{equation}
    \gamma_T := \max_{A\subset \mathcal{D}:|A|=T} \mathbf{I}(\mathbf{y}_A; \mathbf{f}_A),
\end{equation}
where $\mathbf{I}(\mathbf{y}_A; \mathbf{f}_A) = \mathbf{I}(\mathbf{y}_A; f)$, which is the mutual information between $f$ and observations $\mathbf{y}_A = \mathbf{f}_A + \epsilon_A$, defined as:
\begin{equation}
    \mathbf{I}(\mathbf{y}_A; f) = \mathcal{H}(\mathbf{y}_A) - \mathcal{H}(\mathbf{y}_A|f),
\end{equation}
which corresponds to the reduction in entropy $\mathcal{H}$ about $f$ after revealing $\mathbf{y}_A$. 

This leads to an analytic form for the information gain: $\mathbf{I}(\mathbf{y}_A; \mathbf{f}_A) = \frac{1}{2} \text{log}|\mathbf{I} + \sigma^{-2}\mathbf{K}_A|$, where $\mathbf{K}_A = $ since $\mathbf{f}_A = [f(x)]_{x\inA}$, $\epsilon_A \sim \mathcal{N}(0, \sigma^2\mathbf{I})$. 

This result is important, as $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$, so GP-UCB is a \textbf{no regret algorithm}.
\end{comment}

%\vcom{a related paper https://arxiv.org/pdf/1911.01032.pdf which could be used to describe and summarize the regret result}

\subsection{Gaussian Process Bandits for a Time-Varying Function}

%\cite{gp_ucb} were the first to derive a sublinear regret bound for GP-bandit optimization, using the following acquisition function:
% \begin{equation}
%     x_t = \argmax_{x\in \mathcal{D}} \mu_{t-1}(x) + \sqrt{\beta_t} \sigma_{t-1}(x)
% \end{equation}


%However, if we wish to optimize $f_t$, then we need to consider the fact that the function is \texit{changing through time}. This is crucial, as one would expect a neural network to respond differently to  hyperparameters at different stages of training.

% \cite{gp_ucb} present the GP optimization under the bandit setting. They derive the principle way to adapt the decision function for achieving convergence guarantee. For handling our neural network behavior time-varying bandit --

%\vcom{I will write it here}

Following previous works in the GP-bandit literature \cite{gp_ucb}, we model $f_t$ using a Gaussian Process (GP, \cite{RasmussenGP}) which is specified by a mean function $\mu_t : \mathcal{X} \rightarrow \mathbb{R}$ and a kernel (covariance function) $k : \mathcal{D} \times \mathcal{D}  \rightarrow \mathbb{R}$. If $f_t \sim  GP(\mu_t, k)$, then $f_t(x_t)$ is distributed normally $\mathcal{N} (\mu_t(x_t), k(x_t, x_t)) \text{ for all } x_t \in \mathcal{D}$. After we have observed $T$ data points $\{(x_t, f(x_t))\}_{t=1}^T$, the GP posterior belief at new point $x'_t \in \mathcal{D}$, $f_t(x'_t)$ follows  a Gaussian distribution with mean $\mu_t(x')$ and variance $\sigma_t^2(x')$ as: 
% \begin{minipage}[t]{0.48\columnwidth}
% \begin{align}
%  \mu\left(\bx'\right)	=\mathbf{k_{*X}} \left[ \mathbf{K} + \sigma^2_n \idenmat \right]^{-1}\mathbf{y}
%     \label{eq:GPmean}
%     \end{align}
% \end{minipage}%
% \begin{minipage}[t]{0.48\columnwidth}%
% \begin{align}
%     \sigma^{2}\left(\bx_*\right)	=k_{**}-\mathbf{k_{*X}}\left[ \mathbf{K} + \sigma^2_n \idenmat \right]^{-1}\mathbf{k'_{*X}} \label{eq:GPvar}
% \end{align}
% \end{minipage}
\begin{equation}
\label{eqn:mu}
    \mu_t(x') \coloneqq \textbf{k}_t(x')^T(\textbf{K}_t + \sigma^2\textbf{I})^{-1}\mathbf{y}_t
\end{equation}
\begin{equation}
\label{eqn:sig}
    \sigma_t^2(x') \coloneqq k(x', x') - \textbf{k}_t(x')^T(\textbf{K}_t +\sigma^2\textbf{I})^{-1}\textbf{k}_t(x'),
\end{equation}
where $\mathbf{K}_t \coloneqq \{k(x_i, x_j)\}_{i, j=1}^t$ and $\mathbf{k}_t \coloneqq \{k(x_i, x'_t)\}_{i=1}^t$. Equipped with (\ref{eqn:mu}) and (\ref{eqn:sig}), we can select new samples by maximizing an \textit{acquisition function}. 

In order to accurately represent the non-stationary nature of a neural network training process, we cast the problem of optimizing our neural network parameters as time-varying bandit optimization. We follow \cite{bogunovic2016time} to formulate this problem by modelling the reward function under the time-varying setting as follows:
\begin{equation}
     f_1(x) = g_1(x), \; \; f_{t+1}(x) = \sqrt{1-\omega}f_t(x) + \sqrt{\omega}fg_{t+1}(x) \; \: \: \:  \forall t \geq 2,
\end{equation}
where $g_1, g_2, ...$ are independent random functions with $g\sim GP(0, k)$ and $\omega \in[0,1]$ models how the function varies with time, such that if $\omega=0$ we return to GP-UCB and if $\omega=1$ then each evaluation is independent. This model introduces a new hyperparameter ($\omega$), however, we note it can be optimized by maximizing the marginal likelihood for a trivial additional cost compared to the expensive function evaluations (we include additional details on this in the Appendix). This leads to the extensions of Eqs. (\ref{eqn:mu}) and (\ref{eqn:sig}) 
using the new covariance matrix $\Tilde{\textbf{K}}_t = \textbf{K}_t \circ \textbf{K}_t^{\mathrm{time}}$ where $\textbf{K}_t^{\mathrm{time}} = [(1-\omega)^{|i-j|/2}]_{i,j=1}^T$ and $\Tilde{\textbf{k}}_t(x) = \textbf{k}_t \circ \textbf{k}_t^{time}$ with $\textbf{k}_t^{time} = [(1-\omega)^{(T+1-i)/2}]_{i=1}^T$. Here $\circ$ refers to the Hadamard product. 

%We will consider translation invariant kernels $k$ such as the squared exponential (SE) and Matern (see: Section \ref{sec:theory}). 

% This leads to extensions to (\ref{eqn:mu}) and (\ref{eqn:sig}) as follows:
% \begin{equation}
% \label{eqn:tv_mu}
%     \Tilde{\mu}_t(x') \coloneqq \Tilde{\textbf{k}}_t(x')^T(\Tilde{\textbf{K}}_t + \sigma^2\textbf{I})^{-1}\mathbf{y}_t
% \end{equation}
% \begin{equation}
% \label{eqn:tv_sig}
%     \Tilde{\sigma}_t^2(x') \coloneqq k(x', x') - \Tilde{\textbf{k}}_t(x')^T(\Tilde{\textbf{K}}_t +\sigma^2\textbf{I})^{-1}\Tilde{\textbf{k}}_t(x')
% \end{equation}


%This essentially equates to forgetting in a ``smooth'' fashion. 
%Interestingly, despite the additional complexity of a time-varying function, \cite{bogunovic2016time} show this algorithm also achieves sublinear regret: $R_T  \leq \sqrt{C_1 T\beta_T\Tilde{\gamma}_T}+2$ with probability $1-\delta$, where $C_1 = 8/\text{log}(1+\sigma^{-2})$, and $\beta_t$ is chosen appropriately. To see more detail on how this bound is achieved, please see the Appendix, Section \ref{sec:theory} or \cite{bogunovic2016time}. 


% \vcom{We will present the derivative over $\omega$ and put in the supplement for completeness. We may also discuss on how to optimize the block length $\Tilde{N}$. Instead of cross-validation, can we replace it by "optimization". It is basically the same thing and will lead to the same result.}

\subsection{Moving to a Population}

In the PBT setting we need to consider an entire population of agents. This changes the problem from a sequential to a \textit{batch} blackbox optimization problem. This poses an additional challenge, since we must select $x_t$ without full knowledge of all $\{(x_i, y_i)\}_{i=1}^{t-1}$. A key observation in \cite{gp_bucb} is that since a GP's variance (Eqn. \ref{eqn:sig}) does not depend on $y_t$, the acquisition function can  account for incomplete trials by updating the uncertainty at the selected points. Concretely, we define $x_{t,b}$ to be the $b$-th point selected in a batch, after $t$ timesteps. This point may draw on information from $t + (b-1)$ previously selected points. In the single agent, sequential case, we set $B=1$ and recover $t,b = t-1$. Thus, we can select the next sample by maximizing the following acquisition function:
\begin{equation}
\label{eq:gp_bucb_acq}
    x_{{t,b}} = \argmax_{x\in \mathcal{D}} \mu_{{t,1}}(x) + \sqrt{\beta_t} \sigma_{{t,b}}(x)
\end{equation}
for $\beta_t >0$. In Equation \ref{eq:gp_bucb_acq} we have the mean from the previous batch ($\mu_{t,1}(x)$), but can update the uncertainty using our knowledge of the agents currently training ($\sigma_{t,b}(x)$). This significantly reduces redundancy, as the model is able to explore distinct regions of the space.



==> theory_long.tex <==

\section{Theoretical Results}
\label{sec:theory}


We provide the proof for Lemma {\ref{lem:maxreward_minregret}. 
\begin{proof}
We have a reward at the starting iteration $F_1(x_1)$ as a constant that allows us to write the objective function as:
\begin{align}
    F_T(x_T) - F_1(x_1) &=  F_T(x_T) - F_{T-1}(x_{T-1})+  \dots+ F_{3}(x_{3}) - F_{2}(x_{2}) + F_2(x_2) - F_1(x_1) 
    \label{eq:equivalent_reward_regret}
\end{align}

Therefore, maximizing the left of Eq. (\ref{eq:equivalent_reward_regret}) is equivalent to minimizing the cummulative regret as follows:
\begin{align}
    \max \left[ F_T(x_T) - F_1(x_1) \right] &=  \max \sum_{t=1}^T F_t(x_t) - F_{t-1}(x_{t-1})\nonumber \\
    &= \max \sum_{t=1}^T f_t(x_t)\nonumber \\
    & = \min \sum_{t=1}^T r_t(x_t)\nonumber
\end{align}
where we define $f_t(x_t)=F_t(x_t)-F_{t-1}(x_{t-1})$, the regret $r_t=f_t(x^*_t)-f_t(x_t$ and $f_t(x_t^*):= \max_{\forall x} f_t(x)$ is an unknown constant.
%Therefore minimizing regret is equivalent to maximizing final performance.
\end{proof}


\paragraph{Preliminaries} We begin by defining the squared exponential (SE) and Matern (Mat) kernels, for completion: 
\begin{equation}
    k_{SE}(x, x') = \text{exp}\left(- \frac{||x - x'||^2}{2l^2} \right), 
\end{equation}
\begin{equation}
    k_{Mat}(x, x') = \frac{2^{1-\nu}}{\Gamma(\nu)}\left(- \frac{\sqrt{2\nu} ||x - x'||}{l} \right) J_\nu \left(- \frac{\sqrt{2\nu} ||x - x'||}{l} \right),
\end{equation}
where the lengthscale $l>0$, and smoothing parameter $\nu>0$, and $J(\nu)$ and $\Gamma(\nu)$ denote the modified Bessel and Gamma functions, respectively. Our theoretical results will focus on the SE kernel, which was used for all of our experiments. 

\paragraph{Regret.}

A natural performance metric in this context is cumulative regret,
the loss in reward due to not knowing the maximum points of the black-box
function beforehand. Suppose the unknown time-varying function is
$f$, its maximum point at a particular time step $t$ is $\bx_{t}^{*}=\arg\max_{\bx\in D}f_{t}(\bx)$.
For our choice $\bx_{t}$ in iteration $t$, we incur instantaneous
regret $r_{t}=f_{t}\left(\bx_{t}^{*}\right)-f_{t}\left(\bx_{t}\right)$.
The cumulative regret $R_{T}$ after $T$ iterations is the sum of
instantaneous regrets: $R_{T}=\sum_{t=1}^{T}r_{t}$. A desirable asymptotic
property of an algorithm is to be no-regret: $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.
Note that neither $r_{t}$ nor $R_{T}$ are ever revealed to the algorithm.

For the batch setting, we can follow the above to have the batch instantaneous
regret $r_{t}^{B}=\min_{b\le B}r_{t,b}=\min_{b\le B}f_{t}\left(\bx_{t}^{*}\right)\text{\textminus}f_{t}\left(\bx_{t,b}\right)$.

\subsection{Convergence Analysis}

We aim to minimize the cumulative regret $R_{T}$  by sequentially
suggesting an $\bx_{t}$ to be used in each iteration $t$. We shall derive
the upper bound in the cumulative regret and show that it asymptotically
goes to zero as $T$ increases, i.e., $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.

We make the following smoothness assumption to derive the regret bound
of the proposed algorithm.

\textbf{Assumptions.}

We will assume that the kernel $k$ is such that a (strict) subset
of the following statements hold for some $\left(a,b\right)$ and
all $L\ge0$.
\begin{enumerate}
\item The time kernel satisfies $1-k_{time}(t,t')\le\epsilon\left|t-t'\right|$
for some $\epsilon\in\left[0,1\right]$ and for any $t,t'\in\mathcal{T}$.
\item The joint kernel satisfies for $k=1,...,K,$
\begin{align}
\forall L & \ge0,t\le\mathcal{T},p(\sup\left|\frac{\partial f_{t}(\bbeta)}{\partial\bbeta^{(k)}}\right|\le L)\le ae^{-\left(L/b\right)^{2}}.\label{eq:Lipschitz_assumption}
\end{align}
\end{enumerate}
The assumption 1 is achieved by using a time-varying kernel $k_{time}(t,t')=\left(1-\omega\right)^{\frac{|t-t'|}{2}}$
\citep{bogunovic2016time} while assumption 2 is from the smooth functions.
\begin{lemma}
\label{lem:Lipschitz_bound}Let $L_{t}=b\sqrt{\log3da\frac{\pi_{t}}{\delta}})$
where $\sum_{t=1}^{T}\frac{1}{\pi_{t}}=1$, we have with probability
$1-\frac{\delta}{3},$
\begin{align}
\left|f_{t}(\bx)-f_{t}(\bx')\right| & \le L_{t}||\bx-\bx'||_{1},\forall t,\bx,\bx'\in D\label{eq:Lipschitz_Lt}
\end{align}
\end{lemma}

\begin{proof}
Using the Lipschitz assumption in Eq. (\ref{eq:Lipschitz_assumption})
and the union bound over $j=1,...,d$, the event corresponding to
a single time in Eq. (\ref{eq:Lipschitz_Lt}) will hold with the probability
at least $1-da\exp\left(-\frac{L_{t}^{2}}{b^{2}}\right)=1-\frac{\delta}{3\pi_{t}}$.
Taking the union bound over $t$, we get $1-\sum_{t=1}^{T}da\exp\left(-\frac{L_{t}^{2}}{b^{2}}\right)=1-\sum_{t=1}^{T}\frac{\delta}{3\pi_{t}}=1-\frac{\delta}{3}$
since $\sum_{t=1}^{T}\frac{1}{\pi_{t}}=1$.
\end{proof}
Below we define a discretization which serves as a tool for proving
the theorem, but it is not used in the implementation.
\begin{lemma}
\label{lem:bound_discretization}We define a discretization $D_{t}\subset D\subseteq[0,r]^{d}$
of size $(\tau_{t})^{d}$ satisfying $||\bx-\left[\bx\right]_{t}||_{1}\le\frac{d}{\tau_{t}},\forall\bx\in D$
where $\left[\bx\right]_{t}$ denotes the closest point in $D_{t}$
to $\bx$. By choosing $\tau_{t}=\frac{t^{2}}{L_{t}d}=rdbt^{2}\sqrt{\log\left(3da\pi_{t}/\delta\right)}$,
we have
\begin{align*}
|f_{t}(\bx)-f_{t}(\left[\bx\right]_{t})| & \le\frac{1}{t^{2}}
\end{align*}
\end{lemma}

\begin{proof}
Using the discretization assumption and the Lipschitz continuity in
Lem. \ref{lem:Lipschitz_bound}, we have
\begin{align*}
\left|f_{t}(\bx)\text{\textminus}f_{t}(\left[\bx\right]_{t})\right| & \le L_{t}||\bx-\left[\bx\right]_{t}||_{1}\le\frac{L_{t}d}{\tau_{t}}
\end{align*}
By setting $\tau_{t}=\frac{t^{2}}{L_{t}d}$, we have that $\left|f_{t}(\bx)-f_{t}(\left[\bx\right]_{t})\right|\le\frac{1}{t^{2}}$.
\end{proof}
We note that a uniformly-spaced grid suffices to ensure the discretization
holds.
\begin{lemma}
\label{lem:bound_fx_mux}Let $\beta_{t}\ge2\log\frac{3\pi_{t}}{\delta}+2d\log\left(rdbt^{2}\sqrt{\log\frac{3da\pi_{t}}{2\delta}}\right)$
where $\sum_{t=1}^{T}\pi_{t}^{-1}=1$, then with probability at least
$1-\frac{\delta}{3}$, we have
\begin{align*}
|f_{t}(\bx_{t})-\mu_{t}(\bx_{t})|\le & \sqrt{\beta_{t}}\sigma_{t}(\bx_{t}),\forall t,\forall\bx\in\mathcal{D}.
\end{align*}
\end{lemma}

\begin{proof}
We note that conditioned on the outputs $(y_{1},...,y_{t-1})$, the
sampled points $(\bx_{1},...,\bx_{t})$ are deterministic, and $f_{t}(\bx_{t})\sim\mathcal{N}\left(\mu_{t}(\bx_{t}),\sigma_{t}^{2}(\bx_{t})\right)$.
Using Gaussian tail bounds \cite{wainwright2015chapter}, a random
variable $f\sim\mathcal{N}(\mu,\sigma^{2})$ is within $\sqrt{\beta}\sigma$
of $\mu$ with probability at least $1-\exp\left(-\frac{\beta}{2}\right)$.
 Therefore, we first claim that if $\beta_{t}\ge2\log\frac{3\pi_{t}}{\delta}$
then the selected points $\left\{ \bx_{t}\right\} _{t=1}^{T}$ satisfy
the confidence bounds with probability at least $1-\frac{\delta}{3}$
\begin{align}
\left|f_{t}(\bx_{t})-\mu_{t}(\bx_{t})\right| & \le\sqrt{\beta_{t}}\sigma_{t}(\bx_{t}),\forall t.\label{eq:bound_selected_xt}
\end{align}

This is true because the confidence bound for individual $\bx_{t}$
will hold with probability at least $1-\frac{\delta}{3\pi_{t}}$ and
taking union bound over $\forall t$ will lead to $1-\frac{\delta}{3}$.

We show above that the bound is applicable for the selected points
$\left\{ \bx_{t}\right\} _{t=1}^{T}$. To ensure that the bound is
applicable for all points in the domain $D_{t}$ and $\forall t$,
we can set $\beta_{t}\ge2\log\frac{3|D_{t}|\pi_{t}}{\delta}$ where
$\sum_{t=1}^{T}\pi_{t}^{-1}=1$ e.g., $\pi_{t}=\frac{\pi^{2}t^{2}}{6}$
\begin{align}
p(\left|f_{t}\left(\bx_{t}\right)-\mu_{t}\left(\bx_{t}\right)\right| & \le\sqrt{\beta_{t}}\sigma_{t}\left(\bx_{t}\right)\ge1-|D_{t}|\sum_{t=1}^{T}\exp\left(-\beta_{t}/2\right)=1-\frac{\delta}{3}\label{eq:bound_all_Dt}
\end{align}

By discretizing the domain $D_{t}$ in Lem. \ref{lem:bound_discretization},
we have a connection to the cardinality of the domain that $|D_{t}|=(\tau_{t})^{d}=\left(rdbt^{2}\sqrt{\log\left(3da\pi_{t}/\delta\right)}\right)^{d}$.
 Therefore, we need to set $\beta_{t}$ such that both conditions
in Eq. (\ref{eq:bound_selected_xt}) and Eq. (\ref{eq:bound_all_Dt})
are satisfied. We simply take a sum of them and get $\beta_{t}\ge2\log\frac{3\pi_{t}}{\delta}+2d\log\left(rdbt^{2}\sqrt{\log\frac{3da\pi_{t}}{2\delta}}\right)$
.
\end{proof}


\paragraph{Mutual Information:}

The mutual information is one of the key quantities in the original GP-UCB regret bound
\cite{gp_ucb}. We use $TB$ to denote the batch setting where we will run the algorithm over $T$ iterations with a batch size $B$. The mutual information is defined
as $\tilde{\idenmat}(f_{TB};y_{TB})=\frac{1}{2}\log\det\left(\idenmat_{TB}+\sigma_{f}^{-2}\tilde{K}_{TB}\right)$
and the maximum information gain is as $\tilde{\gamma}_{T}:=\max\tilde{\idenmat}({\bf f}_{TB};\by_{TB})$
where ${\bf f}_{TB}:=f_{TB}(\bx_{TB})=\left(f_{t,b}(\bx_{t,b}),...,f_{T,B}(\bx_{T,B})\right),\forall b=1....B,\forall t=t...T$
for the time variant GP $f$. 

To derive the bound over the maximum information gain, we shall split $T\times B$ observations in time steps $\left\{ 1,...,T\right\} $
into $T/\tilde{N}$ blocks of length $\tilde{N}\times B$, such that
within each block the function $f_{i}$ does not vary significantly.
We assume for the time being that $T/\tilde{N}$ is an integer, and
then handle the general case.

We will show that $\tilde{\gamma}_{TB}\le\left(\frac{T}{\tilde{N}B}+1\right)\left(\gamma_{\tilde{N}B}+\sigma_{f}^{-2}\left[\tilde{N}B\right]^{5/2}\omega\right)$
where we note that this bound is tighter than the result presented
in the original paper \citep{bogunovic2016time} ($\tilde{N}^{5/2}\le\tilde{N}^{3}$)
and we have considered noise variance $\sigma_{f}^{2}$ into the analysis.
\begin{lemma}
\label{lem:Mirsky=002019s-theorem}(Mirsky\textquoteright s theorem
{[}\cite{horn2012matrix}, Cor. 7.4.9.3{]}). For any matrices $U$
and $V$ of size $\tilde{N}\times\tilde{N}$, and any unitarily invariant
norm $|||\cdot|||$, we have 
\begin{align*}
|||\textrm{diag}(\lambda_{1}(U),...,\lambda_{\tilde{N}}(U))-\textrm{diag}(\lambda_{1}(V),...,\lambda_{\tilde{N}}(V))||| & \le|||U-V|||
\end{align*}
where $\lambda_{i}(\cdot)$ is the $i$-th largest eigenvalue.
\end{lemma}

\begin{lemma}
\label{lem:bound_MIG_timevarying}Let $\omega$ be the forgetting-remembering
trade-off parameter and consider the kernel for time $1-K_{time}(t,t')\le\omega\left|t-t'\right|$,
we show the bound on the maximum information gain that
\begin{align*}
\tilde{\gamma}_{TB} & \le\left(\frac{T}{\tilde{N}\times B}+1\right)\left(\gamma_{\tilde{N}\times B}+\sigma_{f}^{-2}\left[\tilde{N}\times B\right]^{5/2}\omega\right)
\end{align*}
\end{lemma}

\begin{proof}
We bound the mutual information with time variations by connecting
to the original case (without time variations, \citep{gp_ucb}).
We shall split $T\times B$ observations in time steps $\left\{ 1,...,T\right\} $
into $T/\tilde{N}$ blocks of length $\tilde{N}\times B$, such that
within each block the function $f_{i}$ does not vary significantly.
We assume for the time being that $T/\tilde{N}$ is an integer, and
then handle the general case.

We bound the time-varying maximum information gain for each $i$-th block as $\tilde{\gamma}^{i}:=\max\tilde{\idenmat}^{i}({\bf f}^{i};\by^{i})$
where $\by^{i}=[y_{1},...,y_{\tilde{N}\times B}]$ contains the observations
in the $i$-th blocks and analogous design for ${\bf f}^{i}$, we
write the relevant covariance matrix as
\begin{align*}
\tilde{K}^{i}=K^{i}\circ K_{time}^{i} & =K^{i}+A^{i}
\end{align*}
where $\circ$ denotes the Hadamard product, $K_{time}^{i}=\left[(1-\omega)^{\frac{\left|t-t'\right|}{2}}\right]$,
$A^{i}=K^{i}\circ\left(K_{time}^{i}-\mathbf{1}_{\tilde{N}}\right)$
and $\mathbf{1}_{\tilde{N}}$ is the matrix of one of size $\tilde{N}$.
Each covariance matrix $\tilde{K}^{i},K^{i}$ and $K_{time}^{i}$
will have the same dimension of $\left[\tilde{N}\times B\right]\times\left[\tilde{N}\times B\right]$.
We have each entry in $K^{i}$ is bounded $[0,1]$ and the absolute
value of each entry in $K_{time}^{i}-\mathbf{1}_{\tilde{N}}$ is bounded
by $1-\left(1-\omega\right)^{\frac{\left|i-j\right|}{2}}\le\omega\left|i-j\right|$.

Therefore, we can bound the Frobenius norm of
\begin{align*}
||A^{i}||_{F}\le\sum_{i,j}\left(i-j\right)^{2}\omega^{2}=\frac{1}{6}\left[\tilde{N}\times B\right]^{2}\left(\left[\tilde{N}\times B\right]^{2}-1\right)\omega^{2}\le\left[\tilde{N}\times B\right]^{4}\omega^{2}
\end{align*}
using a standard double summation formula. Let $U=K^{i}+A^{i}$ and
$V=K^{i}$, we define $\Delta_{k}^{i}=\lambda_{k}\left(\tilde{K}^{i}\right)-\lambda_{k}\left(K^{i}\right)$,
we have
\begin{align*}
\sum_{j=1}^{\tilde{N}\times B}\left(\Delta_{j}^{i}\right)^{2} & =\sum_{j=1}^{\tilde{N}\times B}\left(\lambda_{j}\left(\tilde{K}^{i}\right)-\lambda_{j}\left(K^{i}\right)\right)^{2}\\
 & =||diag\left(\lambda_{1}\left(\tilde{K}^{i}\right),...,\lambda_{\tilde{N}\times B}\left(\tilde{K}^{i}\right)\right)-diag\left(\lambda_{1}\left(K^{i}\right),...,\lambda_{\tilde{N}\times B}\left(K^{i}\right)\right)||_{F}^{2} \\
 & \le||A_{\tilde{N}\times B}||_{F}^{2}\le\left[\tilde{N}\times B\right]^{4}\omega^{2}
\end{align*}
where we have utilized Lem. \ref{lem:Mirsky=002019s-theorem}. We
now bound the maximum information gain defined in each block $\tilde{\gamma}^{i}$
and connect it to the standard (time invariant) maximum information
gain $\gamma^{i}$ shown in \cite{gp_ucb}:
\begin{align}
\tilde{\gamma}^{i}= & \frac{1}{2}\log\det\left(\idenmat_{\tilde{N}B\times\tilde{N}B}+\sigma^{-2}\left(\tilde{K}^{i}\right)\right)\nonumber \\
= & \sum_{i=1}^{\tilde{N}\times B}\log\left(1+\sigma^{-2}\lambda_{i}\left(K^{i}+A^{i}\right)\right)=\sum_{i=1}^{\tilde{N}\times B}\log\left(1+\sigma^{-2}\lambda_{i}\left(K^{i}\right)+\sigma^{-2}\Delta_{k}^{i}\right)\nonumber \\
\le & \sum_{i=1}^{\tilde{N}\times B}\log\left(1+\sigma^{-2}\lambda_{i}\left(K^{i}\right)\right)+\sum_{i=1}^{\tilde{N}\times B}\log\left(1+\sigma^{-2}\Delta_{k}^{i}\right)\label{eq:log(1_a_b)}\\
= & \gamma_{\tilde{N}}+\sum_{i=1}^{\tilde{N}\times B}\log\left(1+\sigma^{-2}\lambda_{i}\Delta_{k}^{i}\right)\le\gamma_{\tilde{N}}+\tilde{N}\times B\times\log\left(1+\sigma^{-2}\frac{1}{\tilde{N}\times B}\sum_{i=1}^{\tilde{N}\times B}\Delta_{k}^{i}\right)\label{eq:jensen_delta_i_k}\\
\le & \gamma_{\tilde{N}}+\tilde{N}\times B\times\log\left(1+\sigma^{-2}\left[\tilde{N}\times B\right]^{3/2}\omega\right)\label{eq:MIG_log_sum_delta_ik}\\
\le & \gamma_{\tilde{N}}+\sigma^{-2}\left[\tilde{N}\times B\right]^{5/2}\omega\label{eq:MIG_log(1_x)}
\end{align}
where Eq. (\ref{eq:log(1_a_b)}) is by $\log(1+a+b)\le\log(1+a)+\log(1+b),$
for $a,b>0$. Eq. (\ref{eq:jensen_delta_i_k}) is using Jensen inequality
for $\log\left(1+x\right)$. In Eq. (\ref{eq:MIG_log_sum_delta_ik}),
we utilize the inequality that $\sum_{i=1}^{\tilde{N}\times B}\Delta_{k}^{i}\le\sqrt{\tilde{N}\times B}\sqrt{\sum_{i=1}^{\tilde{N}\times B}\Delta_{k}^{i}}\le\sqrt{\tilde{N}\times B}\left[\tilde{N}\times B\right]^{2}\omega$.
In Eq. (\ref{eq:MIG_log(1_x)}), we utilize $\log(1+x)\le x$ for
$\forall x>-1$.

Using the chain rule for mutual information and the fact that the
noise sequence $\left\{ \epsilon_{t}\right\} _{t=1}^{T}$ where $y_{t}=f_{t}(\bx_{t})+\epsilon_{t}$
is independent, we have
\begin{align*}
\tilde{\idenmat}_{T}\left(f_{T},y_{T}\right) & \le\sum_{i=1}^{T/\tilde{N}}\tilde{\idenmat}^{i}\left({\bf f}^{i};\by^{i}\right)
\end{align*}
Maximizing both sides $\tilde{\gamma}_{T}:=\max\tilde{\idenmat}({\bf f}_{T};\by_{T})$,
we have
\begin{align*}
\tilde{\gamma}_{TB} & \le\sum_{i=1}^{T/\tilde{N}}\tilde{\gamma}^{i}\le\left(\frac{T}{\tilde{N}\times B}+1\right)\left(\gamma_{\tilde{N}}+\sigma_{f}^{-2}\left[\tilde{N}\times B\right]^{5/2}\omega\right)
\end{align*}
where the bounds are similar across blocks $\tilde{\gamma}^{i}\le\gamma_{\tilde{N}\times B}+\frac{1}{\sigma_{f}^{2}}\left[\tilde{N}\times B\right]^{5/2}\omega,\forall i\le\frac{T}{\tilde{N}}$
and the addition of one is for the case when $\frac{T}{\tilde{N}}$
is not an integer.
\end{proof}
In particular, we note that the bound over the maximum information
gain for the time-varying is typically much higher than the standard
(non time-varying setting) due to the fact the time-varying function
$f_{T}$ represents the points of $T$ different random functions,
as opposed to a single function at $T$ different points.

\paragraph{Uncertainty Sampling (US).}

We next derive an upper bound over the maximum information gain obtained
from a batch $\bx_{t,b},\forall b=1,...,B$. In other words, we want
to show that the information gain by our chosen points $\bx_{t,b}$
will not go beyond the chosen points by merely maximizing the uncertainty.
For this, we define an uncertainty sampling (US) scheme which fills
in a batch $\bx_{t,b}^{\textrm{US}}$ by maximizing the GP predictive
variance. Particularly, at iteration $t$, we select $\bx_{t,b}^{\textrm{US}}=\arg\max_{\bx}\sigma_{t}(\bx\mid D_{t,b-1}),\forall b\le B$
and the data set is augmented over time to include the information
of the new point, $D_{t,b}=D_{t,b-1}\cup\bx_{t,b}^{\textrm{US}}$.
We note that we use $\bx_{t,b}^{\textrm{US}}$ to derive the upper
bound, but this is not used by our PB2 algorithm.
\begin{lemma}
\label{lem:bound_UCB_US}Let $\bx^{\textrm{PB2}}$ be the point chosen
by our algorithm and $\bx_{t,b}^{\textrm{US}}$ be the point chosen
by uncertainty sampling (US) by maximizing the GP predictive variance
$\bx_{t,b}^{\textrm{US}}=\arg\max_{\bx\in D}\sigma_{t}(\bx\mid D_{t,b-1}),\forall b=1,...B$
and $D_{t,b}=D_{t,b-1}\cup\bx_{t,b}$, We have
\begin{align*}
\sigma_{t+1,1}\left(\bx_{t+1,1}^{\textrm{PB2}}\right)\le\sigma_{t+1,1}\left(\bx_{t+1,1}^{\textrm{US}}\right) & \le\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right),\forall t\in\left\{ 1,...,T\right\} ,\forall b\in\left\{ 1,...B\right\} 
\end{align*}
\end{lemma}

\begin{proof}
The first inequality is straightforward that the point chosen by uncertainty
sampling will have the highest uncertainty $\sigma_{t+1,1}\left(\bx_{t+1,1}^{\textrm{PB2}}\right)\le\sigma_{t+1,1}\left(\bx_{t+1,1}^{\textrm{US}}\right)=\arg\max_{\bx}\sigma_{t}(\bx\mid D_{t,b-1})$.

The second inequality is obtained by using the principle of \textquotedblleft information
never hurts\textquotedblright{} \cite{Krause_2005Near}, we know that
the GP uncertainty for all locations $\forall\bx$ decreases with
observing a new point. Therefore, the uncertainty at the future iteration
$\sigma_{t+1}$ will be smaller than the uncertainty at the current
iteration $\sigma_{t}$, i.e., $\sigma_{t+1,b}\left(\bx_{t+1,b}^{\textrm{US}}\right)\le\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right),\forall b\le B,\forall t\le T$.
We thus conclude the proof $\sigma_{t+1,1}\left(\bx_{t+1,1}^{\textrm{US}}\right)\le\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right),\forall t\in\left\{ 1,...,T\right\} ,\forall b\in\left\{ 1,...B\right\} $.
\end{proof}
\begin{lemma}
\label{lem:The-sum-variance_UCB}The sum of variances of the points
selected by the our PB2 algorithm $\sigma()$ is bounded by the sum
of variances by uncertainty sampling $\sigma^{\textrm{US}}()$ over
all the selected points divided by $B$ where $B$ is the batch size. Formally, with high probability,
\begin{align*}
\sum_{t=2}^{T}\sigma_{t,1}\left(\bx_{t,1}\right) & \le\frac{1}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)
\end{align*}
\end{lemma}

\begin{proof}
By the definition of uncertainty sampling in Lem. \ref{lem:bound_UCB_US},
we have $\sigma_{t+1,1}\left(\bx_{t+1,1}\right)\le\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right),\forall t\in\left\{ 1,...,T\right\} ,\forall b\in\left\{ 2,...B\right\} $
and $\sigma_{t,1}\left(\bx_{t,1}\right)\le\sigma_{t,1}\left(\bx_{t,1}^{\textrm{US}}\right)$
where $\bx_{t,1}$ is the point chosen by our PB2 and $\bx_{t,1}^{\textrm{US}}$
is from uncertainty sampling. Summing all over $B$, we obtain
\begin{align*}
\sigma_{t,1}\left(\bx_{t,1}\right)+\left(B-1\right)\sigma_{t+1,1}\left(\bx_{t+1,1}\right) & \le\sigma_{t,1}\left(\bx_{t,1}^{\textrm{US}}\right)+\sum_{b=2}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)\\
\sigma_{t,1}\left(\bx_{t,1}\right)+\left(B-1\right)\sigma_{t+1,1}\left(\bx_{t+1,1}\right) & \le\sigma_{t,1}\left(\bx_{t,1}^{\textrm{US}}\right)+\sum_{b=2}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)\\
\sum_{t=1}^{T}\sigma_{t,1}\left(\bx_{t,1}\right)+\left(B-1\right)\sum_{t=1}^{T}\sigma_{t+1,1}\left(\bx_{t+1,1}\right) & \le\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)\,\,\,\,\,\,\,\,\,\,\,\textrm{by}\textrm{\,summing}\thinspace\textrm{over}\thinspace T\\
\sigma_{1,1}\left(\bx_{1,1}\right)+\left(B-1\right)\sigma_{T+1,1}\left(\bx_{T+1,1}\right)+B\sum_{t=2}^{T}\sigma_{t,1}\left(\bx_{t,1}\right) & \le\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)\\
\sum_{t=2}^{T}\sigma_{t,1}\left(\bx_{t,1}\right) & \le\frac{1}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)
\end{align*}
The last equation is obtained because of $\sigma_{1,1}\left(\bx_{1,1}\right)\ge0$
and $\left(B-1\right)\sigma_{T+1,1}\left(\bx_{T+1,1}\right)\ge0$.
\end{proof}
\begin{lemma}
\label{lem:bound_sum_sigma}Let $C_{1}=\frac{32}{\log\left(1+\sigma_{f}^{-2}\right)}$,
$\sigma_{f}^{2}$ be the measurement noise variance and $\tilde{\gamma}_{TB}:=\max\tilde{\idenmat}$
be the maximum information gain of time-varying kernel, we have $\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}^{2}(\bx_{t,b}^{\textrm{US}})\le\frac{C_{1}}{16}\tilde{\gamma}_{TB}$
where $\bx_{t,b}^{\textrm{US}}$ is the point selected by uncertainty
sampling (US).
\end{lemma}

\begin{proof}
We show that $\sigma_{t,b}^{2}(\bx_{t,b}^{\textrm{US}})=\sigma_{f}^{2}\left(\sigma_{f}^{-2}\sigma_{t,b}^{2}(\bx_{t,b}^{\textrm{US}})\right)\le\sigma_{f}^{2}C_{2}\log\left(1+\sigma_{f}^{-2}\sigma_{t,b}^{2}\left(\bx_{t,b}^{\textrm{US}}\right)\right),\forall b\le B,\forall t\le T$
where $C_{2}=\frac{\sigma_{f}^{-2}}{\log\left(1+\sigma_{f}^{-2}\right)}\ge1$
and $\sigma_{f}^{2}$ is the measurement noise variance. We have the
above inequality because $s^{2}\le C_{2}\log\left(1+s^{2}\right)$
for $s\in\left[0,\sigma_{f}^{-2}\right]$ and $\sigma_{f}^{-2}\sigma_{t,b}^{2}\left(\bx_{t,b}^{\textrm{US}}\right)\le\sigma^{-2}k\left(\bx_{t,b}^{\textrm{US}},\bx_{t,b}^{\textrm{US}}\right)\le\sigma_{f}^{-2}$.
We then use Lemma 5.3 of \cite{gp_bucb} to have the
information gain over the points chosen by a time-varying kernel $\tilde{\idenmat}=\frac{1}{2}\sum_{t=1}^{T}\sum_{b=1}^{B}\log\left(1+\sigma_{f}^{-2}\sigma_{t,b}^{2}\left(\bx_{t,b}^{\textrm{US}}\right)\right)$.
Finally, we obtain
\begin{align*}
\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}^{2}(\bx_{t,b}^{\textrm{US}}) & \le\sigma_{f}^{2}C_{2}\sum_{t=1}^{T}\sum_{b=1}^{B}\log\left(1+\sigma_{f}^{-2}\sigma_{t,b}^{2}\left(\bx_{t,b}^{\textrm{US}}\right)\right)=2\sigma_{f}^{2}C_{2}\tilde{\idenmat}=\frac{C_{1}}{16}\tilde{\gamma}_{TB}
\end{align*}
where $C_{1}=\frac{2}{\log\left(1+\sigma_{f}^{-2}\right)}$ and $\tilde{\gamma}_{TB}:=\max\tilde{\idenmat}$
is the definition of maximum information gain given by $T\times B$
data points from a GP for a specific time-varying kernel.
\end{proof}
\begin{theorem}
Let the domain $\mathcal{D}\subset[0,r]^{d}$ be compact and convex
where $d$ is the dimension and suppose that the kernel is such that
$f\sim GP(0,k)$ is almost surely continuously differentiable and
satisfies Lipschitz assumptions for some $a,b$. Fix $\delta\in(0,1)$
and set $\beta_{T}=2\log\frac{\pi^{2}T^{2}}{2\delta}+2d\log rdbT^{2}\sqrt{\log\frac{da\pi^{2}T^{2}}{2\delta}}$.
Defining $C_{1}=32/\log(1+\sigma_{f}^{2})$, the PB2 algorithm satisfies
the following regret bound after $T$ time steps:
\begin{align*}
R_{TB}=\sum_{t=1}^{T}f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t})\le & \sqrt{C_{1}T\beta_{T}\left(\frac{T}{\tilde{N}B}+1\right)\left(\gamma_{\tilde{N}B}+\left[\tilde{N}B\right]^{\frac{5}{2}}\omega\right)}+2
\end{align*}
with probability at least $1-\delta$, the bound is holds for any
$\tilde{N}\in\left\{ 1,...,T\right\} $ and $B\ll T$.
\end{theorem}

\begin{proof}
Let $\bx_{t}^{*}=\arg\max_{\forall\bx}f_{t}(\bx)$ and $\bx_{t,b}$
be the point chosen by our algorithm at iteration $t$ and batch element
$b$, we define the (time-varying) instantaneous regret as $r_{t,b}=f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t,b})$
and the (time-varying) batch instantaneous regret over $B$ points
is as follows
\begin{align}
r_{t}^{B} & =\min_{b\le B}r_{t,b}=\min_{b\le B}f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t,b}),\forall b\le B\nonumber \\
 & \le f_{t}(\bx_{t}^{*})-f_{t}(\bx_{t,1})\nonumber \\
 & \le\text{\ensuremath{\mu_{t}(\bx_{t}^{*})+\sqrt{\beta_{t}}\sigma_{t}(\bx_{t}^{*})+\frac{1}{t^{2}}-f_{t}(\bx_{t,1})}}\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\textrm{by}\,\textrm{Lem}.\,\ref{lem:bound_discretization}\nonumber \\
 & \le\mu_{t}(\bx_{t,1})+\sqrt{\beta_{t}}\sigma_{t}(\bx_{t,1})+\frac{1}{t^{2}}-f_{t}(\bx_{t,1})\label{eq:inequality_beta_t_argmax}\\
 & \le2\sqrt{\beta_{t}}\sigma_{t}(\bx_{t,1})+\frac{1}{t^{2}}\label{eq:bound_rt}
\end{align}
where in Eq. (\ref{eq:inequality_beta_t_argmax}) we have used the
property that $\mu_{t}(\bx_{t,1})+\sqrt{\beta_{t}}\sigma_{t}(\bx_{t,1})\ge\mu_{t}(\bx_{t}^{*})+\sqrt{\beta_{t}}\sigma_{t}(\bx_{t}^{*})$
by the definition of selecting $\bx_{t,1}=\arg\max_{\bx}\mu_{t}(\bx)+\sqrt{\beta_{t}}\sigma_{t}(\bx)$.

Next, we bound the cumulative batch regret as
\begin{align}
R_{TB}=\sum_{t=1}^{T}r_{t}^{B} & \le\sum_{t=1}^{T}\left(2\sqrt{\beta_{t}}\sigma_{t}(\bx_{t,1})+\frac{1}{t^{2}}\right)\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\textrm{by\,Eq.\,(\ref{eq:bound_rt})}\nonumber \\
 & \le2\sqrt{\beta_{T}}\sigma_{1}(\bx_{1,1})+\frac{2\sqrt{\beta_{T}}}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)+\sum_{t=1}^{T}\frac{1}{t^{2}}\,\,\,\,\,\,\,\,\textrm{by}\,\textrm{Lem}.\,\ref{lem:bound_UCB_US}\thinspace\textrm{and\thinspace\ensuremath{\beta_{T}\ge\beta_{t},\forall t}\ensuremath{\le T}}\nonumber \\
 & \le\frac{4\sqrt{\beta_{T}}}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)+\sum_{t=1}^{T}\frac{1}{t^{2}}\label{eq:R_T_two_terms_split}\\
 & \le\frac{4}{B}\sqrt{\beta_{T}\times TB\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}^{2}(\bx_{t,b}^{\textrm{US}})}+2\label{eq:R_T_step2}\\
 & \le\sqrt{C_{1}\frac{T}{B}\beta_{T}\tilde{\gamma}_{TB}}+2\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\thinspace\thinspace\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\thinspace\textrm{by}\thinspace\textrm{Lem}.\thinspace\ref{lem:bound_sum_sigma}\nonumber \\
 & \le\sqrt{C_{1}\frac{T}{B}\beta_{T}\left(\frac{T}{\tilde{N}\times B}+1\right)\left(\gamma_{\tilde{N}B}+\frac{1}{\sigma_{f}^{2}}\left[\tilde{N}\times B\right]^{5/2}\omega\right)}+2.\label{eq:R_T_last_step}
\end{align}
where $C_{1}=32/\log(1+\sigma_{f}^{2})$, $\bx_{t,b}^{\textrm{US}}$
is the point chosen by uncertainty sampling -- used to provide the
upper bound in the uncertainty. In Eq. (\ref{eq:R_T_two_terms_split}),
we take the upper bound by considering two possible cases: either
$1\ge\sigma_{1}(\bx_{1,1})\ge\frac{1}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)$
or $\frac{1}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)\ge\sigma_{1}(\bx_{1,1})$.
It results in $\frac{2}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)\ge\frac{1}{B}\sum_{t=1}^{T}\sum_{b=1}^{B}\sigma_{t,b}\left(\bx_{t,b}^{\textrm{US}}\right)+\sigma_{1}(\bx_{1,1})$.
In Eq. (\ref{eq:R_T_step2}) we have used $\sum_{t=1}^{\infty}\frac{1}{t^{2}}\le\pi^{2}/6\le2$
and $||z||_{1}\le\sqrt{T}||z||_{2}$ for any vector $z\in\mathcal{R}^{T}$.
In Eq. (\ref{eq:R_T_last_step}), we utilize Lem. \ref{lem:bound_MIG_timevarying}.

Finally, given the squared exponential (SE) kernel defined, $\gamma_{\tilde{N}B}^{SE}=\mathcal{O}(\left[\log\tilde{N}B\right]^{d+1})$,
the bound is $R_{TB}\le\sqrt{C_{1}\frac{T}{B}\beta_{T}\left(\frac{T}{\tilde{N}B}+1\right)\left((d+1)\log\left(\tilde{N}B\right)+\frac{1}{\sigma_{f}^{2}}\left[\tilde{N}\times B\right]^{5/2}\omega\right)}+2$
where $\tilde{N}\le T$ and $B\ll T$. We refer to Theorem 5 in \cite{Srinivas_2010Gaussian}
for the bound of other common kernels. We note that this bound $R_{TB}$
in Eq. (\ref{eq:R_T_last_step}) is tighter than in the original paper
\cite{bogunovic2016time} due to the $\tilde{\gamma}_{T}$ derived
in Lem. \ref{lem:bound_MIG_timevarying} (ours $\tilde{N}^{5/2}\le\tilde{N}^{3}$
\cite{bogunovic2016time}).

The regret bound grows sublinearly with the number of iterations $T$,
i.e., $\lim_{T\rightarrow\infty}\frac{R_{TB}}{T}=0$. This bound suggests
that the gap between $f_{t}(\bx_{t})$ and the optimal $f_{t}(\bx_{t}^{*})$
is asymptotically vanished. In addition, our regret bound is tighter
and better with increasing batch size $B$.
\end{proof}

Our theoretical analysis assumed that we know the hyperparameters
of both spatial (length-scale $\sigma_{l}^{2}$ for squared exponential
kernel) and temporal kernel ($\omega$). Having perfect knowledge
of and other hyperparameters is typically not realistic. The GP perspective
allows us to select them in a principled way by maximizing the GP
marginal likelihood.

